A Markov Chain Model for Identifying Changes in Daily Activity Patterns of People Living with Dementia

Malnutrition and dehydration are strongly associated with increased cognitive and functional decline in people living with dementia (PLWD), as well as an increased rate of hospitalisations in comparison to their healthy counterparts. Extreme changes in eating and drinking behaviours can often lead to malnutrition and dehydration, accelerating the progression of cognitive and functional decline and resulting in a marked reduction in quality of life. Unfortunately, there are currently no established methods by which to objectively detect such changes. Here, we present the findings of an extensive quantitative analysis conducted on in-home monitoring data collected from 73 households of PLWD using Internet of Things technologies. The Coronavirus 2019 (COVID-19) pandemic has previously been shown to have dramatically altered the behavioural habits, particularly the eating and drinking habits, of PLWD. Using the COVID-19 pandemic as a natural experiment, we conducted linear mixed-effects modelling to examine changes in mean kitchen activity within a subset of 21 households of PLWD that were continuously monitored for 499 days. We report an observable increase in day-time kitchen activity and a significant decrease in night-time kitchen activity (t(147) = -2.90, p < 0.001). We further propose a novel analytical approach to detecting changes in behaviours of PLWD using Markov modelling applied to remote monitoring data as a proxy for behaviours that cannot be directly measured. Together, these results pave the way to introduce improvements into the monitoring of PLWD in naturalistic settings and for shifting from reactive to proactive care.

==> Text/Supplementary_Information.tex <==
In this section, we provide the supplementary evidence necessary to support our claims.

\subsection{Study Cohort Demographics}

Here we detail the distribution of diagnoses within the study cohort, as well as the variation in year of birth within the study cohort.

\begin{table}[H]
    \centering
    %\scriptsize
    \caption{Diagnoses for the study cohort}
     \begin{tabular}{c| c c c } 
         %\hline
         \toprule
         \textbf{Dementia Type} & \textbf{\%Male} & \textbf{\%Female} & \textbf{\%Total} \\ %[0.5ex] 
         %\hline
         \midrule
         \textbf{Alzheimer's Disease} & 34\% & 36\% & 70\% \\ 
         \textbf{Dementia with Lewy Bodies} & 3\% & 0\% & 3\%  \\
         \textbf{Frontotemporal Dementia} & 1.5\% & 1.5\% & 3\%  \\
         \textbf{Parkinson's Disease Dementia}  & 7\% & 0\% & 7\%  \\ 
         \textbf{Vascular Dementia} & 5\% & 0\% & 5\% \\
         \textbf{Other/Not specified} & 5\% & 7\% & 12\% \\
         %\hline
     \end{tabular}
     \label{tb:dementia_dignoses}
\end{table}

\begin{table}[H]
    \centering
    %\small
     \caption{Year of birth statistics for the study cohort}
     \begin{tabular}{c c| c c c c } 
         \toprule
         %\hline
         \textbf{Total Count} & \textbf{Missing} & \textbf{Mean} & \textbf{Std Dev} & \textbf{Min} & \textbf{Max}\\ %[0.5ex] 
         %\hline
         \midrule
         \textbf{72} & 1(1.5\%) & 1941 & 8.24 & 1927 & 1962 \\ 
         %\hline
     \end{tabular}
     \label{tb:YOB_Stats}
\end{table}

\subsection{Minder Study Inclusion and Exclusion Criteria}

Here we detail the comprehensive criteria by which an individual may be included or excluded from the Minder study.

\subsubsection{Inclusion Criteria}

People living with dementia must meet the following criteria to be included in the Minder study:
\vspace{1em}
\begin{itemize}
    \item Have an established dementia of diagnosis or mild cognitive impairment by specialist assessment.
    \item Be male or female over the age of 50 years old.
    \item Have sufficient functional English to allow completion of the assessment instruments.
    \item If lacking in capacity, participants must have a personal consultee representative.
    \item Have a study partner over the age of 18, with sufficient functional English, willing and able to provide informed consent and who has known the person living with dementia for at least 6 months and is able to attend research assessments with them.
\end{itemize}
\vspace{1em}
\subsubsection{Exclusion criteria}

People living with dementia who meet the following criteria are excluded from the Minder study:
\vspace{1em}
\begin{itemize}
    \item Are in receipt of any investigational drug within a 30-day period prior to consenting.
    \item Have an unstable mental state including severe depression, severe psychosis, agitation, and anxiety whose medication was changed over the last 4 weeks.
    \item Have a severe sensory impairment.
    \item Have active suicidal ideation. 
    \item Require regular elective hospital admission for monitoring of their physical health.
    \item Are receiving treatment for a terminal illness.
    \item Have study partners who are unable to communicate verbally or provide written informed consent.
\end{itemize}
